Selling Information Through Consulting

We consider a monopoly information holder selling information to a budget-constrained decision maker, who may benefit from the seller's information. The decision maker has a utility function that depends on his action and an uncertain state of the world. The seller and the buyer each observe a private signal regarding the state of the world, which may be correlated with each other. The seller's goal is to sell her private information to the buyer and extract maximum possible revenue, subject to the buyer's budget constraints. We consider three different settings with increasing generality, i.e., the seller's signal and the buyer's signal can be independent, correlated, or follow a general distribution accessed through a black-box sampling oracle. For each setting, we design information selling mechanisms which are both optimal and simple in the sense that they can be naturally interpreted, have succinct representations, and can be efficiently computed. Notably, though the optimal mechanism exhibits slightly increasing complexity as the setting becomes more general, all our mechanisms share the same format of acting as a consultant who recommends the best action to the buyer but uses different and carefully designed payment rules for different settings. Each of our optimal mechanisms can be easily computed by solving a single polynomial-size linear program. This significantly simplifies exponential-size LPs solved by the Ellipsoid method in the previous work, which computes the optimal mechanisms in the same setting but without budget limit. Such simplification is enabled by our new characterizations of the optimal mechanism in the (more realistic) budget-constrained setting.

==> app.tex <==
\section{Revelation Principle} \label{app:revelation}
Consider any generic interactive protocol $M$, we construct a mechanism $M'$ that extracts no less revenue, and the buyer truthfully report type $\theta$ and budget $b$ at the root. 

The root of $M'$ is just the buyer node that asks the buyer to report type $\theta$ and $b$. Then we add a subtree $T_{\theta,b}$ below the root for each $(\theta,b)$.  The subtree $T_{\theta,b}$ is just a copy of $M$ in which the seller simulates the optimal strategy of the buyer with type $\theta$ and budget $b$ at each buyer node. So $T_{\theta,b}$ only has seller nodes and transfer nodes. Clearly the buyer will truthfully report $\theta$ and $b$ and the revenue of $M'$ is the same as $M$.


\begin{comment}
\section{Posterior-based LP formulation} \label{app:posterior_LP}
We restate the posterior-based LP formulation from~\cite{Babaioff:2012:OMS:2229012.2229024} in full. They represent a signaling scheme $S(\theta, b)$ by the posterior beliefs formed by an outside observer after receiving the signal produced by this signaling scheme. The outside observer's prior belief of $\omega$ is equal to $\mu(\omega)$. Let $q$ be a possible posterior belief, they define $x_{\theta, b}(q)$ to be the probability that the outside observer's posterior belief equals $q$ after receiving the signal produced by $S(\theta, b)$, and define $t_{\theta, b}(q)$ to be the transfer amount when the signal is realized to the one that gives the outside observer posterior $q$. They also prove that the set of interesting posteriors $Q^*$ is finite, but can be exponentially large. 

The variables of their LP are $x_{\theta, b}(q)$ and $\tilde{t}_{\theta, b}(q) = x_{\theta, b}(q) \cdot t_{\theta, b}(q)$. Their posterior-based LP is then formulated as 
\begin{align}
&\max \ \sum_{\theta, q} (\bm{1}^t D_{\theta,b} q) \cdot \tilde{t}_{\theta,b} \quad  \textrm{s.t. }  \notag\\
 &\sum_q v_{\theta, b}(D_{\theta,b} q) x_{\theta, b}(q) - (\bm{1}^t D_{\theta, b} q) \tilde{t}_{\theta,b}(q) \ge v_{\theta, b}(D_{\theta, b} p), \notag\\
 & \quad \forall \theta,b  \tag{IR}\\
 &\sum_q v_{\theta, b}(D_{\theta,b} q) x_{\theta, b}(q) - (\bm{1}^t D_{\theta, b} q) \tilde{t}_{\theta,b}(q) \notag\\
 & \quad \ge  \sum_q v_{\theta, b}(D_{\theta,b} q) x_{\theta', b'}(q) - (\bm{1}^t D_{\theta,b} q) \tilde{t}_{\theta', b'}(q), \notag\\
 & \quad \forall (\theta', b')\neq (\theta,b) \tag{IC}\\
 & \sum_q x_{\theta, b}(q) q(\omega) = \mu(\omega), \forall \theta,  b, \omega \notag\\
 & \tilde{t}_{\theta,b}(q) \le x_{\theta, b}(q) \cdot b, \ \forall q, \theta, b \notag\\
 & x_{\theta, b}(q) \ge 0. \notag
\end{align}
where $D_{\theta,b}$ is a $|\Omega| \times |\Omega|$ diagonal matrix with $\mu(\theta, b|\omega)$ for all $\omega$ in the diagonal, and $v_{\theta, b}(q)$ is the $(\theta, b)$-buyer's expected utility when $\omega$ follows distribution $q$.



\section{Random Bonus Scheme} \label{app:bonus} 
 
Consider the LP solution $p_{\theta, b}(\cdot)$ and $q_{\theta,b}(\cdot)$ for a fixed $\theta,b$. If there exists some $a,i$ that has $p_{\theta, b}(a, i) = 0$ but $q_{\theta, b}(a,i) < 0$, the transfer amount $t_{\theta, b}(a,i) = q_{\theta, b}(a, i)/p_{\theta, b}(q)$ will be ill-defined. We resolve this problem by adding a ``random bonus scheme'' in parallel with the signaling scheme to simulate $q_{\theta, b}(a,i)$ for these $(a,i)$'s.
 To simplify the notation, we denote the pair $(a_i)$ by $\alpha$. Suppose $\alpha_1, \dots, \alpha_k$ have  $p_{\theta, b}(\alpha) = 0$ but $q_{\theta, b}(\alpha) < 0$. Let $R$ be the minimum number such that $(q_1(\omega)+ \cdots + q_k(\omega))/R \le \mu(\omega)$. WLOG we assume such an $R$ always exists as we can just remove $\omega$ from $\Omega$ if $\mu(\omega) = 0$.  Then this random bonus scheme simulates $t'_{\theta, b}(q)$ as if $x'_{\theta, b}(q) = \frac{1}{R}$, which works as follows:
\begin{itemize}
\item The buyer will receive a random bonus according to his reported type $\theta$ and budget $b$. The amount of the bonus is defined as follows: if the seller's signal is realized to $\omega$, the amount equals $t'_{\theta, b}(q_i)R$ with probability $\frac{q_i(\omega)}{\mu(\omega) R}$ for $i \in [k]$, otherwise the amount equals $0$. 
\end{itemize}

We now prove Theorem~\ref{thm:main}. The theorem is a direct result of Lemma~\ref{lem:corr_poly}. 
Let $\vec{x}'_{\theta, b}$, $\vec{t}'_{\theta, b}$ be an optimal solution in Lemma~\ref{lem:corr_poly}. If the optimal solution has $t'_{\theta, b}(q) = 0$ whenever $x'_{\theta, b}(q) = 0$, then it already represents a valid polynomial-size signaling scheme. Suppose $q_1, \dots, q_k$ are the polynomially many posteriors that have $x'_{\theta, b}(q)>0$. Then we just design $S(\theta, b)$ such that $q_i$ equals the outside observer's posterior belief about $\omega$ at leaf $i$. Specifically, $S(\theta, b)$ has $k$ leaves $s_1, \dots, s_k$ and the transition function $p_{\theta, b}(\omega, s_i)$ (the probability of going to $s_i$ when the seller's signal is realized to $\omega$) satisfies
$$
q_i(\omega) = \frac{\mu(\omega) p_{\theta, b}(\omega, s_i)}{x'_{\theta, b}(q_i)}.
$$
And the transfer amount at leaf $i$ is just $t'_{\theta, b}(q)/x'_{\theta, b}(q)$.
 \end{comment}

\begin{comment}
We prove that for the buyer with type $\theta', b'$, the expected bonus amount when he reports $\theta, b$ will be equal to 
\begin{align*}
& \frac{1}{\mu(\theta', b')}\sum_{i=1}^k (\bm{1}^t D_{\theta', b'} q_i) t'_{\theta, b} (q_i) \\
= & \frac{1}{\mu(\theta', b')} \sum_{i=1}^k \sum_{w} \mu( \theta', b' | \omega) q_i(\omega) t'_{\theta, b}(q_i).
\end{align*}
By our definition, the expected bonus for the buyer with type $\theta', b'$ when he reports $\theta, b$ is equal to 
\begin{align*}
&\sum_{w} \mu(\omega| \theta', b') \sum_{i=1}^k t'_{\theta, b}(q_i)R \cdot \frac{q_i(\omega)}{\mu(\omega) R} \\
=& \sum_{w} \sum_{i=1}^k  \mu(\omega| \theta', b') t'_{\theta, b}(q_i) \cdot \frac{q_i(\omega)}{\mu(\omega) }\\
=& \sum_{w} \sum_{i=1}^k  \frac{\mu(\omega, \theta', b')}{\mu(\theta', b')} \cdot t'_{\theta, b}(q_i) \cdot \frac{q_i(\omega)}{\mu(\omega) }\\
= &  \frac{1}{\mu(\theta', b')}  \sum_{w} \sum_{i=1}^k  \mu( \theta', b' | \omega) \cdot t'_{\theta, b}(q_i) \cdot q_i(\omega).
\end{align*}
which is exactly what we want. 
\end{comment}
